Simulating the universe(s): from cosmic bubble collisions to cosmological observables with numerical relativity

The theory of eternal inflation in an inflaton potential with multiple vacua predicts that our universe is one of many bubble universes nucleating and growing inside an ever-expanding false vacuum. The collision of our bubble with another could provide an important observational signature to test this scenario. We develop and implement an algorithm for accurately computing the cosmological observables arising from bubble collisions directly from the Lagrangian of a single scalar field. We first simulate the collision spacetime by solving Einstein's equations, starting from nucleation and ending at reheating. Taking advantage of the collision's hyperbolic symmetry, simulations are performed with a 1+1-dimensional fully relativistic code that uses adaptive mesh refinement. We then calculate the comoving curvature perturbation in an open Friedmann-Robertson-Walker universe, which is used to determine the temperature anisotropies of the cosmic microwave background radiation. For a fiducial Lagrangian, the anisotropies are well described by a power law in the cosine of the angular distance from the center of the collision signature. For a given form of the Lagrangian, the resulting observational predictions are inherently statistical due to stochastic elements of the bubble nucleation process. Further uncertainties arise due to our imperfect knowledge about inflationary and pre-recombination physics. We characterize observational predictions by computing the probability distributions over four phenomenological parameters which capture these intrinsic and model uncertainties. This represents the first fully-relativistic set of predictions from an ensemble of scalar field models giving rise to eternal inflation, yielding significant differences from previous non-relativistic approximations. Thus, our results provide a basis for a rigorous confrontation of these theories with cosmological data.

==> equations_of_motion.tex <==
\section{Equations of Motion}

The collision space-time possesses an SO(2,1) symmetry, allowing an arbitrary collision to be computed in one space and one time dimension. This follows from the SO(3,1) symmetry of the individual bubbles. One rotational symmetry is broken along the axis separating their centres, but the boost symmetry along this axis is retained. In previous work~\cite{Johnson:2011wt}, the metric 
\begin{equation}\label{eq:generalmetric}
ds^2 =H_F^{-2} \left( -\alpha(\tilde{x}, \tilde{z})^2  d\tilde{z}^2 + a(\tilde{x}, \tilde{z})^2 d\tilde{x}^2 + \tilde{z}^2  \left[ d\chi^2 + \sinh^2 \chi d\phi^2 \right] \right) \, ,
\end{equation}
was used, with the collision space-time parameterized by the two free functions $\alpha(\tilde{x}, \tilde{z})$ and $a(\tilde{x}, \tilde{z})$. Unfortunately, this choice of coordinates is somewhat problematic when evolution for a significant duration of inflation is desired. In pure dS, we have:
\begin{equation}
\alpha = \frac{1}{\sqrt{1+ \tilde{z}^2}}
\end{equation}
and the proper time along a trajectory of constant $x$ is given by:
\begin{equation}
\tau = H_F^{-1} \int_{0}^{z}  \frac{dz}{\sqrt{1+ \tilde{z}^2}} = H_F^{-1} \sinh^{-1} \tilde{z}
\end{equation}
Exponentially long durations of co-ordinate time $z$ must be obtained to simulate over even modest durations in proper time. Evolving over any significant duration of inflation inside of the observation bubble using these coordinates is doomed to failure.

Since the spacetimes we are considering are very close to dS, we define a new time variable $N$:
\begin{equation}
N = \sinh^{-1} z
\end{equation}
and a new pair of metric functions $\bar{\alpha}$ and $\bar{a}$
\begin{equation}
\bar{\alpha} \equiv \alpha \cosh N, \ \ \ \bar{a} \equiv \frac{a}{\cosh N}
\end{equation}
so that the metric becomes
\begin{equation}
ds^2 = - H_F^{-2} \ \bar{\alpha}(\bar{x}, N)^2  dN^2 + H_F^{-2} \cosh^2 N \left( \ \bar{a}(\bar{x}, N)^2 \ d\bar{x}^2 + \tanh^2 N \left[ d\chi^2 + \sinh^2 \chi d\phi^2 \right] \right) \, ,
\end{equation}
In the limit of pure dS, $\bar{\alpha} \rightarrow 1$ and $\bar{a} \rightarrow 1$.

The equation governing the behavior of the scalar field $\varphi$ is
\begin{equation}
\square \varphi =\frac{1}{\sqrt{-g}} \partial_{\mu} \left( \sqrt{-g} g^{\mu \nu} \partial_{\nu} \phi \right) = \partial_{\varphi} V \, .
\end{equation}
Defining the dimensionless variables:
\begin{equation}
\bar{\varphi} = \frac{\varphi}{M_{\rm Pl}}, \ \ \bar{V} = \frac{V}{M_{\rm Pl}^2 H_F^2}
\end{equation}
We reduce this equation to first order form by introducing the variables 
\begin{eqnarray}
\bar{\Phi} &=& \frac{1}{\cosh N} \partial_{\bar{x}} \bar{\varphi} \, , \\
\bar{\Pi} &=& \frac{\bar{a}}{\bar{\alpha}} \left( \partial_N \bar{\varphi} \right) \, .
\end{eqnarray}

In terms of this set of dimensionless variables, the equations of motion are given by:
\begin{equation}
\partial_N \bar{\varphi} = \frac{\bar{\alpha} \bar{\Pi}}{\bar{a}}
\end{equation}
\begin{eqnarray}\label{eq:aN}
\partial_N \bar{a} = - \bar{a} \left( \tanh N + \frac{1}{2 \tanh N} \right) &+& \frac{\bar{a} \bar{\alpha}^2}{2} \left( \frac{1}{\cosh N \sinh N} + 8 \pi \tanh N \ \tilde{V} (\tilde{\phi} ) \right) \nonumber \\ &+& \frac{2 \pi \bar{\alpha}^2 \tanh N}{\bar{a}} \left( \bar{\Phi}^2 + \bar{\Pi}^2 \right)  \, , 
\end{eqnarray}
\begin{eqnarray}\label{eq:alphaN}
\partial_N \bar{\alpha} =  \bar{\alpha} \left( \tanh N + \frac{1}{2 \tanh N} \right) &-& \frac{\alpha^3}{2} \left( \frac{1}{\cosh N \sinh N} + 8 \pi \tanh N \ \tilde{V} (\tilde{\phi} ) \right) \nonumber \\ &+& \frac{2 \pi \bar{\alpha}^3 \tanh N}{\bar{a}^2} \left( \bar{\Phi}^2 + \bar{\Pi}^2 \right)\, , 
\end{eqnarray}
\begin{equation}
\partial_N \bar{\Pi} = - \left(  \tanh N + \frac{2}{\tanh N} \right) \bar{\Pi} + \left( \frac{\bar{\alpha}'}{\bar{a}} - \frac{\bar{a}' \bar{\alpha}}{\bar{a}^2} \right) \frac{\bar{\Phi}}{\cosh N} + \frac{\bar{\alpha}}{\bar{a} \cosh N} \partial_{\bar{x}} \bar{\Phi} -\bar{a} \bar{\alpha} \ \frac{d\bar{V}}{d\bar{\varphi}}
\end{equation}
\begin{equation}
\partial_N \bar{\Phi} = - \tanh N \ \bar{\Phi} + \frac{1}{\cosh N}  \partial_{\bar{x}} \left( \frac{\bar{\alpha}}{\bar{a}} \bar{\Pi}  \right) 
\end{equation}
We also have the constraint equation:
\begin{equation}
\partial_{\bar{x}} \bar{\alpha} = \frac{4 \pi \sinh N \ \bar{\alpha}^2 \bar{\Phi} \bar{\Pi} }{\bar{a}}
\end{equation}

==> initial_conditions.tex <==
\section{Initial Conditions}
The initial conditions for colliding bubbles are determined following the methods outlined in Ref.~\cite{Johnson:2011wt}. First, the scalar field and metric profile for individual bubbles is found. At an early time, the field as a function of the proper distance from a fiducial point can be determined, and mapped to the simulation coordinates used in Eq.~\ref{eq:simulationmetric}. For individual bubbles, profiles for the field and metric functions can be determined perturbatively. The initial conditions for two sufficiently widely separated bubbles can then be obtained by adding the profiles for single bubbles.
\subsection{Individual bubbles} 
The profile for each bubble is determined by the Coleman de Luccia instanton~\cite{Coleman:1977py,Coleman:1980aw}, a compact solution to the Euclidean equations of motion with metric
\begin{equation}\label{eq:CDLmetric}
ds^2 = dt^2 + \rho(t)^2 d\Omega_3^2 \, .
\end{equation}
The metric function $\rho(t)$ has two zeros at $t=0$ and $t=t_\mathrm{max}$, and evolves according to the Euclidean Friedmann and field equations
\begin{eqnarray}
\frac{d^2 \rho}{dt^2} &=& - \frac{8 \pi}{3 M_{\rm Pl}^2} \rho \ \left( \left( \frac{d \varphi}{dt} \right)^2 + V(\varphi) \right) \, . \label{eq:instanton} \\
\frac{d^2 \varphi}{dt^2} &=& -\frac{3}{\rho} \frac{d \rho }{dt} \frac{d \varphi}{dt} + \frac{dV}{d \varphi}. \label{eq:eucfield}
\end{eqnarray}
The CDL instanton is a non-singular solution to the equations of motion that interpolates between the basins of attraction of the true and false vacua. A review of CDL instantons and their construction can be found in e.g. Ref.~\cite{Banks:2002nm}. 

In general, numerical methods must be used to construct the CDL instanton. We have modified the Cosmo Transitions code~\cite{Wainwright:2011kj} to include the effects of gravity.  [{\bf Max, describe this in more detail......}]. 


==> metric_reconstruction.tex <==
%\section{Metric Reconstruction}




\subsection{Constraint equations in synchronous gauge}

To zeroth order in perturbations, the metric functions should satisfy the Friedmann equations:
\begin{equation}
\left( \frac{\partial_t a}{a} \right)^2 = \frac{8 \pi G_N}{3} \left( \frac{(\partial_t \phi^{(\rm no \ coll)} )^2}{2} + V \right) + \frac{1}{a^2}
\end{equation}
At first order in perturbations, we get a constraint from the $t-x$ component of the Einstein equation:
\begin{equation}
2 \partial_t \partial_x \Psi^{(\rm syn)} = 8 \pi G_N \partial_t \phi^{(\rm no \ coll)} \partial_x \delta \phi^{\rm (syn)}
\end{equation}
yielding
\begin{equation}
2 \partial_t \left( D^{(\rm syn)} + \frac{1}{4} E_{\rm xx} \right) = 8 \pi G_N \partial_t \phi^{(\rm no \ coll)} \ \delta \phi^{\rm (syn)}
\end{equation}
In principle, we should include the contribution from curvature here, but the time derivative kills this term at linear order.

Going to second order, we have:
\begin{equation}
2 \partial_t \partial_x \Psi^{(\rm syn)} + 4 \partial_x \Psi^{(\rm syn)} \partial_t \Psi^{(\rm syn)} + 4 \Psi^{(\rm syn)} \partial_t \partial_x \Psi^{(\rm syn)} - \partial_x \Psi^{(\rm syn)} \partial_t \partial^2_x E = 8 \pi G_N \left( \partial_t \phi^{(\rm no \ coll)} \partial_x \delta \phi^{\rm (syn)} +  \partial_t \delta \phi^{\rm (syn)} \partial_x \delta \phi^{\rm (syn)}  \right)    
\end{equation}
Now, we must include the curvature term: $\Psi^{(\rm syn)} \rightarrow D^{(\rm syn)} + D^{(\rm curv)} + \frac{1}{4} E_{\rm xx}$. Substituting, we obtain:
\begin{eqnarray}
8 \pi G_N \left( \partial_t \phi^{(\rm no \ coll)} \partial_x \delta \phi^{\rm (syn)} +  \partial_t \delta \phi^{\rm (syn)} \partial_x \delta \phi^{\rm (syn)}  \right)   & = & 2 \partial_t \partial_x \left( D^{(\rm syn)} + \frac{1}{4} E_{\rm xx} \right) \nonumber \\ 
&+& 4 \partial_x \left(  D^{(\rm syn)} + D^{(\rm curv)} + \frac{1}{4} E_{\rm xx} \right) \partial_t \left(  D^{(\rm syn)} + \frac{1}{4} E_{\rm xx} \right) \nonumber \\
&+& 4 \left(  D^{(\rm syn)} + D^{(\rm curv)} + \frac{1}{4} E_{\rm xx} \right) \partial_t \partial_x  \left(  D^{(\rm syn)}  + \frac{1}{4} E_{\rm xx} \right) \nonumber \\
&-& \partial_x \left(  D^{(\rm syn)} + D^{(\rm curv)} + \frac{1}{4} E_{\rm xx} \right) \frac{3}{2} \partial_t E_{xx} 
\end{eqnarray}
Collecting terms:
\begin{eqnarray}
8 \pi G_N \left( \partial_t \phi^{(\rm no \ coll)} \partial_x \delta \phi^{\rm (syn)} +  \partial_t \delta \phi^{\rm (syn)} \partial_x \delta \phi^{\rm (syn)}  \right)   & = & 
\left( 2 - x^2 + 4D^{(\rm syn)} + E_{xx} \right) \partial_x \partial_t \left( D^{(\rm syn)} +  \frac{1}{4} E_{\rm xx} \right) \nonumber \\
&-& 2 x \partial_t D^{(\rm syn)} + \frac{x}{4} \partial_t E_{xx} \nonumber \\
&+& \partial_x  D^{(\rm syn)} \left( 4 \partial_t  D^{(\rm syn)} - \frac{1}{2} \partial_t  E_{xx} \right) \nonumber \\
&+& \partial_x E_{xx} \left( \partial_t  D^{(\rm syn)} - \frac{1}{8} \partial_t  E_{xx} \right)
\end{eqnarray}


